Cached and Confused: Web Cache Deception in the Wild

Web cache deception (WCD) is an attack proposed in 2017, where an attacker tricks a caching proxy into erroneously storing private information transmitted over the Internet and subsequently gains unauthorized access to that cached data. Due to the widespread use of web caches and, in particular, the use of massive networks of caching proxies deployed by content distribution network (CDN) providers as a critical component of the Internet, WCD puts a substantial population of Internet users at risk. We present the first large-scale study that quantifies the prevalence of WCD in 340 high-profile sites among the Alexa Top 5K. Our analysis reveals WCD vulnerabilities that leak private user data as well as secret authentication and authorization tokens that can be leveraged by an attacker to mount damaging web application attacks. Furthermore, we explore WCD in a scientific framework as an instance of the path confusion class of attacks, and demonstrate that variations on the path confusion technique used make it possible to exploit sites that are otherwise not impacted by the original attack. Our findings show that many popular sites remain vulnerable two years after the public disclosure of WCD. Our empirical experiments with popular CDN providers underline the fact that web caches are not plug & play technologies. In order to mitigate WCD, site operators must adopt a holistic view of their web infrastructure and carefully configure cache settings appropriate for their applications.

==> revision.tex <==
\appendix
\section{Revision Notes}

We thank the USENIX Security 2019 Program Committee for their helpful feedback
on the previous iteration of our paper. Here, we explain how we addressed the
major revision items in this revision, and discuss further changes pertaining to
reviewers' minor comments and asks for clarification. As we also disclosed in
Sec.~\ref{section:ethics}, we would like to point out that one of the authors is
affiliated with a major CDN provider, and is hands-on involved with their
customers' cache configurations and defenses against WCD. We also hope to
clarify in this revision some of our decisions that may have seemed arbitrary,
but were in fact based on our domain expertise.

\paragraph{``(1) refrain from merely using Google OAuth sites.''; ``(3) test all different vectors outlined both in §2.3 and §5.1.''}
These two changes were unanimously requested by reviewers, and therefore they
constitute our most significant update in this revision. We repositioned the
paper to present two measurement studies that follow our methodology. The first
study we describe in Sec.~\ref{sec:analysis} is our original experiment, showing
the impact of the basic WCD on a seed pool of 295 sites, and providing a deep
analysis of leaked sensitive data types. Sec.~\ref{sec:advanced_path_confusion}
now presents an entirely new follow-up experiment where we apply all five
variations of WCD on \emph{all} sites. Furthermore, we expand our seed pool to
include all previous 295 sites, and an additional 45 sites that \emph{do not}
use Google OAuth, for a total of 340. This second experiment demonstrates that
variations on WCD can be severely damaging, as we were able to exploit 11 sites
that are not impacted by the basic attack. In total, our experiments identified
37 vulnerable sites, and we have reached out to them in accordance with the
responsible disclosure procedure we explained in Sec.~\ref{section:ethics}. As
of this writing, many site operators have gotten in touch with us, and 12 sites
fixed their vulnerabilities. We have updated the rest of the paper (e.g.,
introduction, abstract) to reflect these updates.

\paragraph{``(2) cluster URLs based on their content/structure (and URL structure, if need be) and only test once URL per cluster if sensitive information is contained.''}

We revised the clustering methodology used in our new experiment to make it more
efficient for our purposes, and less resource-intensive on our
targets. Specifically, we only selected and exploited a page among the first 500
pages when there is at least one marker in the content, whereas previously we
exploited all first 500 pages. Furthermore, based on the results of the previous
experiment showing that all discovered vulnerabilities were exploitable by an
unauthenticated user, we performed the new experiment only with an
unauthenticated attacker account.

Note that we still refrain from content-based clustering of pages, but group
URLs based on their structure. To repeat our rebuttal for the original reviews,
path confusion requires exploiting the particular URL parsing, interpretation,
and serving logic in a web application. When grouping URLs in our experiment,
our goal is to cluster together pages that are highly-likely to be generated
from the same template, and served in the same way, executing similar code
paths. Clustering pages based on their content is not an effective strategy for
this purpose: Content similarity does not necessarily mean that URLs and path
interpretation mechanisms are similar---a necessary prerequisite for path confusion as
aforementioned. Therefore, this could lead to us missing many potential
vulnerable pages, or otherwise bias our results in unpredictable ways.

We added these details and clarifications to our methodology for the reader.

\paragraph{``(4) launch a victim's visit on one machine and then launch an attacker's visit from another machine located far from the victim (maybe one in the US and the other in EU accessed via VPN). Can you still obtain the victim's private information?''; ``(5) launch a victim's visit on one machine, and then launch an attacker's visit after 1-2 days. Can you still obtain the victim's private information?''; ``(6) setup websites that are hosted by these CDNs and see themselves whether these CDNs do cache contents regardless of what your own website says.''}

We performed additional experiments to test the practical implications of
different cache setups and presented our findings in the \emph{Impact of the
  Cache Setup} subsection in Sec.~\ref{sec:advanced_path_confusion}. These
include tests performed from different geographical locations to see the impact
of CDNs' client-to-edge server mappings, and time-delayed experiments to see the
impact of cache TTLs. Please see the corresponding section for details.

We would like to clarify that these experiments are useful for demonstrating the
practical challenges of launching a WCD attack, but these are not new findings;
the sources we cite throughout this paper document these challenges and their
workarounds (e.g., attackers often connect to CDN edge servers using IP
addresses to bypass dynamic DNS mapping).

We realize that this change does not head-on address all reviewer
expectations. Specifically, our experiment does not aim to, and is not designed
to untangle the proxy/cache/CDN configuration of targeted sites. Instead, the
purpose of our paper is to demonstrate the prevalence and impact of WCD and its
variations. Understanding what cache technology is faulty is an extremely
ambitious task, and drawing on our internal view of the ecosystem, an open
research problem major CDNs and their customers struggle with. For instance, we
have performed a case study (not discussed in the paper, due to our legal
obligations to the involved CDN and its customers) and looked at cache
configurations of 10 targets in our seed pool. These configuration files
contained on the order of 10,000 lines of code governing the cache behavior for
different web properties. What is more, it is standard practice for CDN
customers to chain technologies from multiple CDN vendors, and combine these
with their own proxy mechanisms that external researchers do not have visibility
into.

In light of the above, creating CDN accounts to test for CDN behavior is also
not possible, as most commercial CDNs are not plug \& play technologies, but
require writing extensive configurations (i.e., 10,000 lines of code as we
describe above). A ``default behavior'' to test does not exist. However, these
are not relevant for our purposes. The fact remains that major CDN providers
provide options to bypass cache header directives (e.g.,
\cite{akamai_cacheoverride,cloudflare_cacheoverride}), and our results
demonstrate that popular sites indeed use these features.

\paragraph{Safety vs. Security.}
Multiple reviewers discuss whether CDNs and other MITM-proxy technologies should
respect cache headers, and in particular, \emph{Review 381C} states as a major
weakness of our paper that ``I will not blame the website; instead, I would
think this as a vulnerability of the cache.''

We agree that websites are not to blame, but we also strongly object to blaming
any other technology involved in this vulnerability. Our \emph{Discussion and
  Conclusion} section (i.e., Sec.~\ref{sec:conclusion}) discusses this point at
length. Specifically, WCD is widely considered a systems \emph{safety}
problem. In other words, there are no individual insecure or faulty components,
everything works as intended (CDN users have important use cases where they opt
to ignore cache headers), and there is no single entity to blame; in fact,
passing blame is considered counterproductive to handling safety issues in the
safety engineering literature. Instead, the problem stems from multiple
\emph{individually secure components} interacting in hazardous ways, causing an
\emph{accident}. Safety thinking is one of the major points we would like to
emphasize in this paper, and therefore we discuss it extensively both in the
introduction and conclusion. We also refer our readers to one of the seminal
texts in this field by Nancy G. Leveson, ``Engineering a Safer
World~\cite{safety}.'' We also point out that safety thinking is the actual
concrete approach that major CDN vendors adopt when handling WCD and similar
attacks.

\paragraph{``You should at least cite Lekies et al USENIX 2015 on dynamic JavaScript.''}
We cited this paper, and also expanded the related work section with the recent
HTTP Desync and Smuggling attacks~\cite{httpdesync}.

\paragraph{Impact of sub-domain enumeration and robots.txt on target sites.}
We expanded Sec.~\ref{section:ethics} to address these issues.

\paragraph{``How did the crawler handle the user sessions?''}
We expanded the methodology to clarify that crawlers periodically reauthenticate
and avoid logout links.

\paragraph{``You only try your caching attack with a .css file''}
We expanded our methodology to better motivate this choice. In short, style
sheets are ideal candidates as they are highly likely to come with all modern
websites. While images are also good candidates, many CDN technologies include
image transformation technologies that dynamically resize/reencode images as
opposed to statically caching them, making them less likely to enable a
successful attack. Besides, picking one image format over others is an arbitrary
decision, and a comprehensive exploration of the problem would require using
payloads for many possible image, multimedia, and container formats. We choose
.css files as the optimal payload under these constraints.



==> tables/exploitability.tex <==
\begin{table}[t]
    \caption{Attack scenarios.}
    \label{tab:analysis:exploitability}
	\footnotesize
	
    \begin{tabular}{lcc}
    \toprule
    \textbf{Attack Scenario} &
    \textbf{Vulnerable} &
    \textbf{Exploitable} \\
    
    \midrule
Session Hijacking & 6 & 6  \\
Cross-site Request Forgery & 5 & 4 \\
oAuth Redirection URI CSRF & 1 & 1 \\
Cross-site Script Inclusion (XSSI) & N/A & 2 \\
    \bottomrule
    \end{tabular}
\end{table}

